SlowLab: Benchmarking Autonomous AI Agents on a Year of Experiments They Cannot Undo

AI agents are increasingly proposed as autonomous experimenters, yet the benchmarks that test them mostly offer cheap experiments that answer at once. Experiments in physical facilities are different: they take months, occupy scarce equipment and cannot be undone. We present SlowLab, a benchmark in which an agent runs a one-year campaign in four simulated greenhouse compartments on a site whose crop, facility and prices are hidden. The agent decides when to plant which climate policy, whether to stop a crop and which measurements to read while crops grow, and at the end recommends one policy, which a private evaluator scores in weather the agent never saw. In a preregistered study on 48 unseen sites, three low-cost language-model agents ended near a standard grower setting and clearly below a Bayesian-optimisation baseline that starts from that setting. They ran the facility as two synchronous batches, so measurements taken during the season never changed what they planted, and these measurements improved no method's result. Letting other methods re-read the evidence a campaign had collected did not yield significantly better recommendations, which points to where the models start and which experiments they try. Code is released under the MIT license.

==> generated/numbers.tex <==
% Generated by scripts/make_paper_numbers.py; do not edit.
\makeatletter
\newcommand{\res}[1]{\@ifundefined{res@#1}{\textbf{??#1}}{\@nameuse{res@#1}}}
\@namedef{res@E1.deepseek.hi}{$-$4.00}
\@namedef{res@E1.deepseek.lo}{$-$6.91}
\@namedef{res@E1.deepseek.mde}{2.69}
\@namedef{res@E1.deepseek.mean}{$-$5.60}
\@namedef{res@E1.deepseek.p}{$<$0.001}
\@namedef{res@E1.deepseek.sd}{5.07}
\@namedef{res@E1.glm.hi}{$-$2.41}
\@namedef{res@E1.glm.lo}{$-$5.34}
\@namedef{res@E1.glm.mde}{2.80}
\@namedef{res@E1.glm.mean}{$-$3.99}
\@namedef{res@E1.glm.p}{$<$0.001}
\@namedef{res@E1.glm.sd}{5.28}
\@namedef{res@E1.mimo.hi}{$-$3.23}
\@namedef{res@E1.mimo.lo}{$-$6.39}
\@namedef{res@E1.mimo.mde}{3.03}
\@namedef{res@E1.mimo.mean}{$-$4.71}
\@namedef{res@E1.mimo.p}{$<$0.001}
\@namedef{res@E1.mimo.sd}{5.71}
\@namedef{res@E2.baseline.hi}{+0.18}
\@namedef{res@E2.baseline.lo}{$-$1.71}
\@namedef{res@E2.baseline.mde}{1.79}
\@namedef{res@E2.baseline.mean}{$-$0.72}
\@namedef{res@E2.baseline.p}{0.44}
\@namedef{res@E2.baseline.sd}{3.37}
\@namedef{res@E2.deepseek.hi}{+0.29}
\@namedef{res@E2.deepseek.lo}{$-$1.07}
\@namedef{res@E2.deepseek.mde}{1.30}
\@namedef{res@E2.deepseek.mean}{$-$0.30}
\@namedef{res@E2.deepseek.p}{0.81}
\@namedef{res@E2.deepseek.sd}{2.45}
\@namedef{res@E2.glm.hi}{+0.11}
\@namedef{res@E2.glm.lo}{$-$1.61}
\@namedef{res@E2.glm.mde}{1.63}
\@namedef{res@E2.glm.mean}{$-$0.76}
\@namedef{res@E2.glm.p}{0.39}
\@namedef{res@E2.glm.sd}{3.08}
\@namedef{res@E2.mimo.hi}{+0.49}
\@namedef{res@E2.mimo.lo}{$-$1.88}
\@namedef{res@E2.mimo.mde}{2.06}
\@namedef{res@E2.mimo.mean}{$-$0.34}
\@namedef{res@E2.mimo.p}{0.81}
\@namedef{res@E2.mimo.sd}{3.88}
\@namedef{res@E3.deepseek.hi}{+0.46}
\@namedef{res@E3.deepseek.lo}{$-$1.83}
\@namedef{res@E3.deepseek.mean}{$-$0.57}
\@namedef{res@E3.deepseek.on.baseline}{+0.22}
\@namedef{res@E3.deepseek.on.deepseek}{+0.40}
\@namedef{res@E3.deepseek.on.glm}{$-$2.25}
\@namedef{res@E3.deepseek.on.mimo}{$-$1.00}
\@namedef{res@E3.deepseek.p}{0.71}
\@namedef{res@E3.glm.hi}{+0.19}
\@namedef{res@E3.glm.lo}{$-$1.73}
\@namedef{res@E3.glm.mean}{$-$0.64}
\@namedef{res@E3.glm.on.baseline}{$-$0.90}
\@namedef{res@E3.glm.on.deepseek}{+0.09}
\@namedef{res@E3.glm.on.glm}{$-$1.45}
\@namedef{res@E3.glm.on.mimo}{$-$0.93}
\@namedef{res@E3.glm.p}{0.51}
\@namedef{res@E3.gp.hi}{+1.74}
\@namedef{res@E3.gp.lo}{+0.26}
\@namedef{res@E3.gp.mean}{+0.85}
\@namedef{res@E3.gp.on.baseline}{$-$0.00}
\@namedef{res@E3.gp.on.deepseek}{+1.67}
\@namedef{res@E3.gp.on.glm}{+0.84}
\@namedef{res@E3.gp.on.mimo}{+0.55}
\@namedef{res@E3.gp.p}{0.064}
\@namedef{res@E3.mimo.hi}{+0.60}
\@namedef{res@E3.mimo.lo}{$-$1.28}
\@namedef{res@E3.mimo.mean}{$-$0.40}
\@namedef{res@E3.mimo.on.baseline}{+0.78}
\@namedef{res@E3.mimo.on.deepseek}{+0.37}
\@namedef{res@E3.mimo.on.glm}{$-$1.93}
\@namedef{res@E3.mimo.on.mimo}{$-$1.35}
\@namedef{res@E3.mimo.p}{0.71}
\@namedef{res@agc.co2.limit}{361}
\@namedef{res@agc.co2.rmse}{211.8}
\@namedef{res@agc.rh.limit}{8.50}
\@namedef{res@agc.rh.rmse}{9.983}
\@namedef{res@agc.temp.limit}{2.04}
\@namedef{res@agc.temp.rmse}{2.579}
\@namedef{res@calls.deepseek}{62}
\@namedef{res@calls.glm}{61}
\@namedef{res@calls.mimo}{84}
\@namedef{res@calls.original}{19874}
\@namedef{res@calls.repair}{1260}
\@namedef{res@calls.total}{21134}
\@namedef{res@campaigns}{480}
\@namedef{res@cost.deepseek}{0.079}
\@namedef{res@cost.glm}{0.048}
\@namedef{res@cost.mimo}{0.052}
\@namedef{res@dm.0.05.deepseek}{$-$7.06}
\@namedef{res@dm.0.05.glm}{$-$5.58}
\@namedef{res@dm.0.05.mimo}{$-$6.61}
\@namedef{res@dm.0.07.deepseek}{$-$4.56}
\@namedef{res@dm.0.07.glm}{$-$2.86}
\@namedef{res@dm.0.07.mimo}{$-$3.36}
\@namedef{res@evaluations}{2880}
\@namedef{res@fb.deepseek.campaigns}{96}
\@namedef{res@fb.deepseek.predictor}{0.9}
\@namedef{res@fb.deepseek.reads}{6.1}
\@namedef{res@fb.deepseek.sameschedule}{48}
\@namedef{res@fb.deepseek.stops}{0}
\@namedef{res@fb.deepseek.waitpct}{94}
\@namedef{res@fb.glm.campaigns}{96}
\@namedef{res@fb.glm.predictor}{1.8}
\@namedef{res@fb.glm.reads}{5.9}
\@namedef{res@fb.glm.sameschedule}{61}
\@namedef{res@fb.glm.stops}{1}
\@namedef{res@fb.glm.waitpct}{98}
\@namedef{res@fb.mimo.campaigns}{96}
\@namedef{res@fb.mimo.predictor}{3.6}
\@namedef{res@fb.mimo.reads}{7.7}
\@namedef{res@fb.mimo.sameschedule}{49}
\@namedef{res@fb.mimo.stops}{0}
\@namedef{res@fb.mimo.waitpct}{100}
\@namedef{res@fb.stops.total}{1}
\@namedef{res@formaterr.deepseek}{1.3}
\@namedef{res@formaterr.glm}{1}
\@namedef{res@formaterr.mimo}{12}
\@namedef{res@gaindiff.deepseek.baseline.hi}{+1.75}
\@namedef{res@gaindiff.deepseek.baseline.lo}{$-$0.97}
\@namedef{res@gaindiff.deepseek.baseline.mean}{+0.42}
\@namedef{res@gaindiff.deepseek.baseline.p}{0.72}
\@namedef{res@gaindiff.deepseek.glm.hi}{+1.48}
\@namedef{res@gaindiff.deepseek.glm.lo}{$-$0.59}
\@namedef{res@gaindiff.deepseek.glm.mean}{+0.46}
\@namedef{res@gaindiff.deepseek.glm.p}{0.71}
\@namedef{res@gaindiff.deepseek.mimo.hi}{+1.49}
\@namedef{res@gaindiff.deepseek.mimo.lo}{$-$1.06}
\@namedef{res@gaindiff.deepseek.mimo.mean}{+0.04}
\@namedef{res@gaindiff.deepseek.mimo.p}{0.96}
\@namedef{res@gaindiff.glm.baseline.hi}{+1.39}
\@namedef{res@gaindiff.glm.baseline.lo}{$-$1.28}
\@namedef{res@gaindiff.glm.baseline.mean}{$-$0.03}
\@namedef{res@gaindiff.glm.baseline.p}{0.96}
\@namedef{res@gaindiff.glm.mimo.hi}{+1.26}
\@namedef{res@gaindiff.glm.mimo.lo}{$-$1.66}
\@namedef{res@gaindiff.glm.mimo.mean}{$-$0.42}
\@namedef{res@gaindiff.glm.mimo.p}{0.72}
\@namedef{res@gaindiff.mimo.baseline.hi}{+1.60}
\@namedef{res@gaindiff.mimo.baseline.lo}{$-$1.22}
\@namedef{res@gaindiff.mimo.baseline.mean}{+0.39}
\@namedef{res@gaindiff.mimo.baseline.p}{0.72}
\@namedef{res@kernel.crops}{788}
\@namedef{res@kernel.cross.interaction}{0.80}
\@namedef{res@kernel.cross.product}{0.53}
\@namedef{res@kernel.groups}{118}
\@namedef{res@kernel.rmse.interaction}{11.3}
\@namedef{res@kernel.rmse.mean}{18.3}
\@namedef{res@kernel.rmse.refit}{19.7}
\@namedef{res@learn.deepseek.hi}{+4.13}
\@namedef{res@learn.deepseek.lo}{+1.06}
\@namedef{res@learn.deepseek.mean}{+2.65}
\@namedef{res@learn.deepseek.p}{0.018}
\@namedef{res@learn.glm.hi}{+2.42}
\@namedef{res@learn.glm.lo}{+0.06}
\@namedef{res@learn.glm.mean}{+1.27}
\@namedef{res@learn.glm.p}{0.13}
\@namedef{res@learn.mimo.hi}{+3.60}
\@namedef{res@learn.mimo.lo}{+0.50}
\@namedef{res@learn.mimo.mean}{+2.05}
\@namedef{res@learn.mimo.p}{0.064}
\@namedef{res@mean.baseline.endpoint}{34.34}
\@namedef{res@mean.baseline.full}{33.62}
\@namedef{res@mean.deepseek.endpoint}{28.31}
\@namedef{res@mean.deepseek.full}{28.02}
\@namedef{res@mean.deepseek.initial}{25.36}
\@namedef{res@mean.fixed.reference}{29.34}
\@namedef{res@mean.glm.endpoint}{30.38}
\@namedef{res@mean.glm.full}{29.62}
\@namedef{res@mean.glm.initial}{28.35}
\@namedef{res@mean.mimo.endpoint}{29.24}
\@namedef{res@mean.mimo.full}{28.90}
\@namedef{res@mean.mimo.initial}{26.86}
\@namedef{res@observe.deepseek}{10.4}
\@namedef{res@observe.glm}{12.6}
\@namedef{res@observe.mimo}{11.7}
\@namedef{res@orig.E1.deepseek.hi}{$-$1.80}
\@namedef{res@orig.E1.deepseek.lo}{$-$4.35}
\@namedef{res@orig.E1.deepseek.mde}{2.38}
\@namedef{res@orig.E1.deepseek.mean}{$-$3.09}
\@namedef{res@orig.E1.deepseek.p}{$<$0.001}
\@namedef{res@orig.E1.deepseek.sd}{4.48}
\@namedef{res@orig.E1.glm.hi}{$-$0.03}
\@namedef{res@orig.E1.glm.lo}{$-$2.93}
\@namedef{res@orig.E1.glm.mde}{2.72}
\@namedef{res@orig.E1.glm.mean}{$-$1.43}
\@namedef{res@orig.E1.glm.p}{0.29}
\@namedef{res@orig.E1.glm.sd}{5.14}
\@namedef{res@orig.E1.mimo.hi}{$-$0.72}
\@namedef{res@orig.E1.mimo.lo}{$-$3.57}
\@namedef{res@orig.E1.mimo.mde}{2.73}
\@namedef{res@orig.E1.mimo.mean}{$-$2.05}
\@namedef{res@orig.E1.mimo.p}{0.044}
\@namedef{res@orig.E1.mimo.sd}{5.14}
\@namedef{res@orig.E2.baseline.hi}{+0.38}
\@namedef{res@orig.E2.baseline.lo}{$-$0.46}
\@namedef{res@orig.E2.baseline.mde}{0.81}
\@namedef{res@orig.E2.baseline.mean}{$-$0.04}
\@namedef{res@orig.E2.baseline.p}{1.00}
\@namedef{res@orig.E2.baseline.sd}{1.52}
\@namedef{res@orig.E2.deepseek.hi}{+0.29}
\@namedef{res@orig.E2.deepseek.lo}{$-$1.07}
\@namedef{res@orig.E2.deepseek.mde}{1.30}
\@namedef{res@orig.E2.deepseek.mean}{$-$0.30}
\@namedef{res@orig.E2.deepseek.p}{1.00}
\@namedef{res@orig.E2.deepseek.sd}{2.44}
\@namedef{res@orig.E2.glm.hi}{+0.03}
\@namedef{res@orig.E2.glm.lo}{$-$1.49}
\@namedef{res@orig.E2.glm.mde}{1.45}
\@namedef{res@orig.E2.glm.mean}{$-$0.71}
\@namedef{res@orig.E2.glm.p}{0.32}
\@namedef{res@orig.E2.glm.sd}{2.73}
\@namedef{res@orig.E2.mimo.hi}{+0.65}
\@namedef{res@orig.E2.mimo.lo}{$-$1.74}
\@namedef{res@orig.E2.mimo.mde}{2.09}
\@namedef{res@orig.E2.mimo.mean}{$-$0.19}
\@namedef{res@orig.E2.mimo.p}{1.00}
\@namedef{res@orig.E2.mimo.sd}{3.93}
\@namedef{res@orig.E3.deepseek.hi}{$-$0.39}
\@namedef{res@orig.E3.deepseek.lo}{$-$2.66}
\@namedef{res@orig.E3.deepseek.mean}{$-$1.48}
\@namedef{res@orig.E3.deepseek.on.baseline}{$-$2.39}
\@namedef{res@orig.E3.deepseek.on.deepseek}{+0.40}
\@namedef{res@orig.E3.deepseek.on.glm}{$-$2.28}
\@namedef{res@orig.E3.deepseek.on.mimo}{$-$1.52}
\@namedef{res@orig.E3.deepseek.p}{0.041}
\@namedef{res@orig.E3.glm.hi}{$-$0.39}
\@namedef{res@orig.E3.glm.lo}{$-$2.15}
\@namedef{res@orig.E3.glm.mean}{$-$1.22}
\@namedef{res@orig.E3.glm.on.baseline}{$-$1.64}
\@namedef{res@orig.E3.glm.on.deepseek}{+0.09}
\@namedef{res@orig.E3.glm.on.glm}{$-$1.55}
\@namedef{res@orig.E3.glm.on.mimo}{$-$1.54}
\@namedef{res@orig.E3.glm.p}{0.031}
\@namedef{res@orig.E3.gp.hi}{+1.52}
\@namedef{res@orig.E3.gp.lo}{+0.03}
\@namedef{res@orig.E3.gp.mean}{+0.70}
\@namedef{res@orig.E3.gp.on.baseline}{+0.46}
\@namedef{res@orig.E3.gp.on.deepseek}{+1.67}
\@namedef{res@orig.E3.gp.on.glm}{+1.07}
\@namedef{res@orig.E3.gp.on.mimo}{$-$0.55}
\@namedef{res@orig.E3.gp.p}{0.13}
\@namedef{res@orig.E3.mimo.hi}{$-$0.90}
\@namedef{res@orig.E3.mimo.lo}{$-$3.55}
\@namedef{res@orig.E3.mimo.mean}{$-$2.10}
\@namedef{res@orig.E3.mimo.on.baseline}{$-$3.14}
\@namedef{res@orig.E3.mimo.on.deepseek}{+0.37}
\@namedef{res@orig.E3.mimo.on.glm}{$-$2.99}
\@namedef{res@orig.E3.mimo.on.mimo}{$-$1.73}
\@namedef{res@orig.E3.mimo.p}{0.013}
\@namedef{res@orig.dm.0.05.deepseek}{$-$4.45}
\@namedef{res@orig.dm.0.05.glm}{$-$2.92}
\@namedef{res@orig.dm.0.05.mimo}{$-$3.83}
\@namedef{res@orig.dm.0.07.deepseek}{$-$2.12}
\@namedef{res@orig.dm.0.07.glm}{$-$0.37}
\@namedef{res@orig.dm.0.07.mimo}{$-$0.78}
\@namedef{res@orig.gaindiff.deepseek.baseline.hi}{+0.51}
\@namedef{res@orig.gaindiff.deepseek.baseline.lo}{$-$1.23}
\@namedef{res@orig.gaindiff.deepseek.baseline.mean}{$-$0.26}
\@namedef{res@orig.gaindiff.deepseek.baseline.p}{0.73}
\@namedef{res@orig.gaindiff.deepseek.glm.hi}{+1.28}
\@namedef{res@orig.gaindiff.deepseek.glm.lo}{$-$0.48}
\@namedef{res@orig.gaindiff.deepseek.glm.mean}{+0.41}
\@namedef{res@orig.gaindiff.deepseek.glm.p}{0.58}
\@namedef{res@orig.gaindiff.deepseek.mimo.hi}{+1.34}
\@namedef{res@orig.gaindiff.deepseek.mimo.lo}{$-$1.27}
\@namedef{res@orig.gaindiff.deepseek.mimo.mean}{$-$0.11}
\@namedef{res@orig.gaindiff.deepseek.mimo.p}{0.87}
\@namedef{res@orig.gaindiff.glm.baseline.hi}{+0.21}
\@namedef{res@orig.gaindiff.glm.baseline.lo}{$-$1.57}
\@namedef{res@orig.gaindiff.glm.baseline.mean}{$-$0.67}
\@namedef{res@orig.gaindiff.glm.baseline.p}{0.26}
\@namedef{res@orig.gaindiff.glm.mimo.hi}{+1.10}
\@namedef{res@orig.gaindiff.glm.mimo.lo}{$-$1.74}
\@namedef{res@orig.gaindiff.glm.mimo.mean}{$-$0.52}
\@namedef{res@orig.gaindiff.glm.mimo.p}{0.70}
\@namedef{res@orig.gaindiff.mimo.baseline.hi}{+0.72}
\@namedef{res@orig.gaindiff.mimo.baseline.lo}{$-$2.07}
\@namedef{res@orig.gaindiff.mimo.baseline.mean}{$-$0.15}
\@namedef{res@orig.gaindiff.mimo.baseline.p}{0.87}
\@namedef{res@orig.learn.deepseek.hi}{+4.13}
\@namedef{res@orig.learn.deepseek.lo}{+1.06}
\@namedef{res@orig.learn.deepseek.mean}{+2.65}
\@namedef{res@orig.learn.deepseek.p}{0.013}
\@namedef{res@orig.learn.glm.hi}{+2.44}
\@namedef{res@orig.learn.glm.lo}{+0.11}
\@namedef{res@orig.learn.glm.mean}{+1.32}
\@namedef{res@orig.learn.glm.p}{0.070}
\@namedef{res@orig.learn.mimo.hi}{+3.72}
\@namedef{res@orig.learn.mimo.lo}{+0.65}
\@namedef{res@orig.learn.mimo.mean}{+2.19}
\@namedef{res@orig.learn.mimo.p}{0.031}
\@namedef{res@orig.mean.baseline.endpoint}{31.14}
\@namedef{res@orig.mean.baseline.full}{31.10}
\@namedef{res@orig.mean.deepseek.endpoint}{28.31}
\@namedef{res@orig.mean.deepseek.full}{28.01}
\@namedef{res@orig.mean.deepseek.initial}{25.36}
\@namedef{res@orig.mean.fixed.reference}{29.34}
\@namedef{res@orig.mean.glm.endpoint}{30.38}
\@namedef{res@orig.mean.glm.full}{29.67}
\@namedef{res@orig.mean.glm.initial}{28.35}
\@namedef{res@orig.mean.mimo.endpoint}{29.24}
\@namedef{res@orig.mean.mimo.full}{29.05}
\@namedef{res@orig.mean.mimo.initial}{26.86}
\@namedef{res@orig.radius.15.mean}{38.83}
\@namedef{res@orig.radius.15.sd}{2.45}
\@namedef{res@orig.radius.25.mean}{37.45}
\@namedef{res@orig.radius.25.sd}{3.41}
\@namedef{res@orig.radius.35.mean}{35.57}
\@namedef{res@orig.radius.35.sd}{4.06}
\@namedef{res@orig.radius.fixed}{34.92}
\@namedef{res@orig.radius.selected}{15}
\@namedef{res@orig.radius.v3.mean}{27.86}
\@namedef{res@orig.range.E1.abs.hi}{3.09}
\@namedef{res@orig.range.E1.abs.lo}{1.43}
\@namedef{res@orig.range.E1.hi}{$-$1.43}
\@namedef{res@orig.range.E1.lo}{$-$3.09}
\@namedef{res@orig.range.E2.abs.hi}{0.71}
\@namedef{res@orig.range.E2.abs.lo}{0.04}
\@namedef{res@orig.range.E2.hi}{$-$0.04}
\@namedef{res@orig.range.E2.lo}{$-$0.71}
\@namedef{res@orig.range.E3.gp.llm.hi}{+1.67}
\@namedef{res@orig.range.E3.llm.hi}{$-$1.22}
\@namedef{res@orig.range.E3.llm.lo}{$-$2.10}
\@namedef{res@orig.range.E3.llm.p.hi}{0.041}
\@namedef{res@orig.range.E3.llm.p.lo}{0.013}
\@namedef{res@orig.range.gaindiff.p.lo}{0.26}
\@namedef{res@orig.range.initial.hi}{28.35}
\@namedef{res@orig.range.initial.lo}{25.36}
\@namedef{res@orig.range.learn.hi}{+2.65}
\@namedef{res@orig.range.learn.lo}{+1.32}
\@namedef{res@orig.range.llm.full.heat.hi}{160}
\@namedef{res@orig.range.llm.full.heat.lo}{146}
\@namedef{res@orig.range.llm.full.light.hi}{91}
\@namedef{res@orig.range.llm.full.light.lo}{78}
\@namedef{res@orig.ref.baseline.vsfixed}{+1.54}
\@namedef{res@orig.ref.deepseek.vsfixed}{$-$3.04}
\@namedef{res@orig.ref.err.hi}{2.05}
\@namedef{res@orig.ref.err.lo}{1.63}
\@namedef{res@orig.ref.glm.vsfixed}{$-$0.11}
\@namedef{res@orig.ref.headroom}{7.56}
\@namedef{res@orig.ref.mimo.vsfixed}{$-$4.66}
\@namedef{res@orig.ref.sites}{8}
\@namedef{res@orig.res.baseline.endpoint.co2}{13.7}
\@namedef{res@orig.res.baseline.endpoint.heat}{130}
\@namedef{res@orig.res.baseline.endpoint.light}{118}
\@namedef{res@orig.res.baseline.full.co2}{13.7}
\@namedef{res@orig.res.baseline.full.heat}{129}
\@namedef{res@orig.res.baseline.full.light}{119}
\@namedef{res@orig.res.deepseek.endpoint.co2}{13.0}
\@namedef{res@orig.res.deepseek.endpoint.heat}{158}
\@namedef{res@orig.res.deepseek.endpoint.light}{89}
\@namedef{res@orig.res.deepseek.full.co2}{13.2}
\@namedef{res@orig.res.deepseek.full.heat}{160}
\@namedef{res@orig.res.deepseek.full.light}{91}
\@namedef{res@orig.res.deepseek.initial.co2}{15.7}
\@namedef{res@orig.res.deepseek.initial.heat}{172}
\@namedef{res@orig.res.deepseek.initial.light}{116}
\@namedef{res@orig.res.fixed.reference.co2}{14.1}
\@namedef{res@orig.res.fixed.reference.heat}{139}
\@namedef{res@orig.res.fixed.reference.light}{109}
\@namedef{res@orig.res.glm.endpoint.co2}{14.2}
\@namedef{res@orig.res.glm.endpoint.heat}{147}
\@namedef{res@orig.res.glm.endpoint.light}{84}
\@namedef{res@orig.res.glm.full.co2}{13.8}
\@namedef{res@orig.res.glm.full.heat}{148}
\@namedef{res@orig.res.glm.full.light}{81}
\@namedef{res@orig.res.glm.initial.co2}{13.9}
\@namedef{res@orig.res.glm.initial.heat}{140}
\@namedef{res@orig.res.glm.initial.light}{100}
\@namedef{res@orig.res.mimo.endpoint.co2}{13.5}
\@namedef{res@orig.res.mimo.endpoint.heat}{146}
\@namedef{res@orig.res.mimo.endpoint.light}{78}
\@namedef{res@orig.res.mimo.full.co2}{13.4}
\@namedef{res@orig.res.mimo.full.heat}{146}
\@namedef{res@orig.res.mimo.full.light}{78}
\@namedef{res@orig.res.mimo.initial.co2}{14.8}
\@namedef{res@orig.res.mimo.initial.heat}{149}
\@namedef{res@orig.res.mimo.initial.light}{107}
\@namedef{res@orig.secondary.family}{17}
\@namedef{res@orig.ueff.0.deepseek}{$-$2.28}
\@namedef{res@orig.ueff.0.glm}{$-$1.48}
\@namedef{res@orig.ueff.0.mimo}{$-$0.06}
\@namedef{res@orig.ueff.0.rankchange}{changed}
\@namedef{res@orig.ueff.4.deepseek}{+0.70}
\@namedef{res@orig.ueff.4.glm}{+1.72}
\@namedef{res@orig.ueff.4.mimo}{+3.23}
\@namedef{res@orig.ueff.4.rankchange}{changed}
\@namedef{res@orig.ueff.main.deepseek}{$-$2.14}
\@namedef{res@orig.ueff.main.glm}{$-$1.40}
\@namedef{res@orig.ueff.main.mimo}{+0.08}
\@namedef{res@orig.ueff.sites}{16}
\@namedef{res@orig.vsfixed.baseline.hi}{+2.25}
\@namedef{res@orig.vsfixed.baseline.lo}{+1.31}
\@namedef{res@orig.vsfixed.baseline.mean}{+1.76}
\@namedef{res@orig.vsfixed.baseline.p}{$<$0.001}
\@namedef{res@orig.vsfixed.deepseek.hi}{$-$0.28}
\@namedef{res@orig.vsfixed.deepseek.lo}{$-$2.35}
\@namedef{res@orig.vsfixed.deepseek.mean}{$-$1.33}
\@namedef{res@orig.vsfixed.deepseek.p}{0.045}
\@namedef{res@orig.vsfixed.glm.hi}{+1.56}
\@namedef{res@orig.vsfixed.glm.lo}{$-$0.91}
\@namedef{res@orig.vsfixed.glm.mean}{+0.33}
\@namedef{res@orig.vsfixed.glm.p}{0.73}
\@namedef{res@orig.vsfixed.mimo.hi}{+0.98}
\@namedef{res@orig.vsfixed.mimo.lo}{$-$1.67}
\@namedef{res@orig.vsfixed.mimo.mean}{$-$0.29}
\@namedef{res@orig.vsfixed.mimo.p}{0.77}
\@namedef{res@parity.identical}{bit-identical}
\@namedef{res@pilot.baseline.repeatsd}{2.75}
\@namedef{res@pilot.bo.repeatsd}{11.84}
\@namedef{res@pilot.bo.vsfixed}{$-$7.30}
\@namedef{res@pilot.llm.repeatsd.hi}{6.30}
\@namedef{res@pilot.llm.repeatsd.lo}{4.20}
\@namedef{res@radius.15.mean}{36.38}
\@namedef{res@radius.15.sd}{6.20}
\@namedef{res@radius.25.mean}{37.79}
\@namedef{res@radius.25.sd}{6.33}
\@namedef{res@radius.35.mean}{38.13}
\@namedef{res@radius.35.sd}{7.53}
\@namedef{res@radius.fixed}{34.92}
\@namedef{res@radius.selected}{35}
\@namedef{res@radius.v3.mean}{27.86}
\@namedef{res@range.E1.abs.hi}{5.60}
\@namedef{res@range.E1.abs.lo}{3.99}
\@namedef{res@range.E1.hi}{$-$3.99}
\@namedef{res@range.E1.lo}{$-$5.60}
\@namedef{res@range.E2.abs.hi}{0.76}
\@namedef{res@range.E2.abs.lo}{0.30}
\@namedef{res@range.E2.hi}{$-$0.30}
\@namedef{res@range.E2.lo}{$-$0.76}
\@namedef{res@range.E3.gp.llm.hi}{+1.67}
\@namedef{res@range.E3.llm.hi}{$-$0.40}
\@namedef{res@range.E3.llm.lo}{$-$0.64}
\@namedef{res@range.E3.llm.p.hi}{0.71}
\@namedef{res@range.E3.llm.p.lo}{0.51}
\@namedef{res@range.fb.predictor.hi}{3.6}
\@namedef{res@range.fb.predictor.lo}{0.9}
\@namedef{res@range.fb.reads.hi}{7.7}
\@namedef{res@range.fb.reads.lo}{5.9}
\@namedef{res@range.fb.waitpct.hi}{100}
\@namedef{res@range.fb.waitpct.lo}{94}
\@namedef{res@range.gaindiff.p.lo}{0.71}
\@namedef{res@range.initial.hi}{28.35}
\@namedef{res@range.initial.lo}{25.36}
\@namedef{res@range.learn.hi}{+2.65}
\@namedef{res@range.learn.lo}{+1.27}
\@namedef{res@range.llm.full.heat.hi}{160}
\@namedef{res@range.llm.full.heat.lo}{147}
\@namedef{res@range.llm.full.light.hi}{91}
\@namedef{res@range.llm.full.light.lo}{78}
\@namedef{res@range.mde.hi}{3.03}
\@namedef{res@range.mde.lo}{1.30}
\@namedef{res@ref.baseline.vsfixed}{+4.83}
\@namedef{res@ref.deepseek.vsfixed}{$-$3.04}
\@namedef{res@ref.err.hi}{2.05}
\@namedef{res@ref.err.lo}{1.63}
\@namedef{res@ref.glm.vsfixed}{$-$0.70}
\@namedef{res@ref.headroom}{7.56}
\@namedef{res@ref.mimo.vsfixed}{$-$5.13}
\@namedef{res@ref.sites}{8}
\@namedef{res@repair.audits}{288}
\@namedef{res@repair.baseline}{192}
\@namedef{res@repair.branches}{26}
\@namedef{res@repair.branches.deepseek}{3}
\@namedef{res@repair.branches.glm}{16}
\@namedef{res@repair.branches.mimo}{7}
\@namedef{res@repair.e3packets}{23}
\@namedef{res@repair.evaluations}{654}
\@namedef{res@repair.failed}{7}
\@namedef{res@repair.live}{988}
\@namedef{res@repair.replayed}{559}
\@namedef{res@repair.socketparity}{identical}
\@namedef{res@res.baseline.endpoint.co2}{15.1}
\@namedef{res@res.baseline.endpoint.heat}{95}
\@namedef{res@res.baseline.endpoint.light}{99}
\@namedef{res@res.baseline.full.co2}{15.8}
\@namedef{res@res.baseline.full.heat}{95}
\@namedef{res@res.baseline.full.light}{116}
\@namedef{res@res.deepseek.endpoint.co2}{13.0}
\@namedef{res@res.deepseek.endpoint.heat}{158}
\@namedef{res@res.deepseek.endpoint.light}{89}
\@namedef{res@res.deepseek.full.co2}{13.3}
\@namedef{res@res.deepseek.full.heat}{160}
\@namedef{res@res.deepseek.full.light}{91}
\@namedef{res@res.deepseek.initial.co2}{15.7}
\@namedef{res@res.deepseek.initial.heat}{172}
\@namedef{res@res.deepseek.initial.light}{116}
\@namedef{res@res.fixed.reference.co2}{14.1}
\@namedef{res@res.fixed.reference.heat}{139}
\@namedef{res@res.fixed.reference.light}{109}
\@namedef{res@res.glm.endpoint.co2}{14.2}
\@namedef{res@res.glm.endpoint.heat}{147}
\@namedef{res@res.glm.endpoint.light}{84}
\@namedef{res@res.glm.full.co2}{13.9}
\@namedef{res@res.glm.full.heat}{148}
\@namedef{res@res.glm.full.light}{81}
\@namedef{res@res.glm.initial.co2}{13.9}
\@namedef{res@res.glm.initial.heat}{140}
\@namedef{res@res.glm.initial.light}{100}
\@namedef{res@res.mimo.endpoint.co2}{13.5}
\@namedef{res@res.mimo.endpoint.heat}{146}
\@namedef{res@res.mimo.endpoint.light}{78}
\@namedef{res@res.mimo.full.co2}{13.4}
\@namedef{res@res.mimo.full.heat}{147}
\@namedef{res@res.mimo.full.light}{78}
\@namedef{res@res.mimo.initial.co2}{14.8}
\@namedef{res@res.mimo.initial.heat}{149}
\@namedef{res@res.mimo.initial.light}{107}
\@namedef{res@secondary.family}{17}
\@namedef{res@sites}{48}
\@namedef{res@spend.campaigns}{17.27}
\@namedef{res@spend.original}{17.42}
\@namedef{res@spend.repair}{1.29}
\@namedef{res@spend.total}{18.70}
\@namedef{res@ueff.0.deepseek}{$-$4.34}
\@namedef{res@ueff.0.glm}{$-$3.47}
\@namedef{res@ueff.0.mimo}{$-$2.11}
\@namedef{res@ueff.0.rankchange}{unchanged}
\@namedef{res@ueff.4.deepseek}{$-$2.19}
\@namedef{res@ueff.4.glm}{$-$0.90}
\@namedef{res@ueff.4.mimo}{+0.30}
\@namedef{res@ueff.4.rankchange}{changed}
\@namedef{res@ueff.main.deepseek}{$-$5.23}
\@namedef{res@ueff.main.glm}{$-$4.31}
\@namedef{res@ueff.main.mimo}{$-$3.04}
\@namedef{res@ueff.sites}{16}
\@namedef{res@valid.evalerr.paired}{0.76}
\@namedef{res@valid.replay.evals}{8}
\@namedef{res@valid.replay.identical}{bit-identical}
\@namedef{res@valid.trace.campaigns}{12}
\@namedef{res@valid.trace.identical}{bit-identical}
\@namedef{res@vsfixed.baseline.hi}{+4.84}
\@namedef{res@vsfixed.baseline.lo}{+3.62}
\@namedef{res@vsfixed.baseline.mean}{+4.28}
\@namedef{res@vsfixed.baseline.p}{$<$0.001}
\@namedef{res@vsfixed.deepseek.hi}{$-$0.28}
\@namedef{res@vsfixed.deepseek.lo}{$-$2.35}
\@namedef{res@vsfixed.deepseek.mean}{$-$1.32}
\@namedef{res@vsfixed.deepseek.p}{0.064}
\@namedef{res@vsfixed.glm.hi}{+1.59}
\@namedef{res@vsfixed.glm.lo}{$-$0.92}
\@namedef{res@vsfixed.glm.mean}{+0.28}
\@namedef{res@vsfixed.glm.p}{0.75}
\@namedef{res@vsfixed.mimo.hi}{+0.85}
\@namedef{res@vsfixed.mimo.lo}{$-$1.81}
\@namedef{res@vsfixed.mimo.mean}{$-$0.44}
\@namedef{res@vsfixed.mimo.p}{0.72}
\makeatother

